Universal effective couplings of the three-dimensional $n$-vector model and field theory

We calculate the universal ratios $R_{2k}$ of renormalized coupling constants $g_{2k}$ entering the critical equation of state for the generalized Heisenberg (three-dimensional $n$-vector) model. Renormalization group (RG) expansions of $R_8$ and $R_{10}$ for arbitrary $n$ are found in the four-loop and three-loop approximations respectively. Universal octic coupling $R_8^*$ is estimated for physical values of spin dimensionality $n = 0, 1, 2, 3$ and for $n = 4,...64$ to get an idea about asymptotic behavior of $R_8^*$. Its numerical values are obtained by means of the resummation of the RG series and within the pseudo-$\varepsilon$ expansion approach. Regarding $R_{10}$ our calculations show that three-loop RG and pseudo-$\varepsilon$ expansions possess big and rapidly growing coefficients for physical values of $n$ what prevents getting fair numerical estimates.

==> houc.tex <==
@article{PhysRevB.15.1552,
  author = {Baker, George A.},
  journal = {Phys. Rev. B},
  volume = {15},
  issue = {3},
  pages = {1552},
  year = {1977},
}


@article{PhysRevLett.39.95,
  author = {Le Guillou, J. C. and Zinn-Justin, J.},
  journal = {Phys. Rev. Lett.},
  volume = {39},
  issue = {2},
  pages = {95},
  year = {1977},
}

@article{PhysRevB.17.1365,
  author = {Baker, George A. and Nickel, Bernie G. and Meiron, Daniel I.},
  journal = {Phys. Rev. B},
  volume = {17},
  issue = {3},
  pages = {1365},
  year = {1978},
}

@article{PhysRevB.21.3976,
  author = {Le Guillou, J. C. and Zinn-Justin, J.},
  journal = {Phys. Rev. B},
  volume = {21},
  issue = {9},
  pages = {3976},
  year = {1980},
}

@article{PhysRevB.41.402,
  author = {Bagnuls, C. and Bervillier, C.},
  journal = {Phys. Rev. B},
  volume = {41},
  issue = {1},
  pages = {402},
  year = {1990},
}


@article{PhysRevLett.68.3674,
  author = {Bender, Carl M. and Boettcher, Stefan and Lipatov, Lev},
  journal = {Phys. Rev. Lett.},
  volume = {68},
  issue = {25},
  pages = {3674},
  year = {1992},
}

@article{PhysRevD.48.4919,
  author = {Bender, Carl M. and Boettcher, Stefan},
  journal = {Phys. Rev. D},
  volume = {48},
  issue = {10},
  pages = {4919},
  year = {1993},
}

@article{TETRADIS1994541,
journal = "Nucl. Phys. B",
volume = "422",
pages = "541",
year = "1994",
author = "N. Tetradis and C. Wetterich",
}

@article{PhysRevD.51.1875,
  author = {Bender, Carl M. and Boettcher, Stefan},
  journal = {Phys. Rev. D},
  volume = {51},
  issue = {4},
  pages = {1875},
  year = {1995},
}

@article{REISZ199577,
journal = "Phys. Lett. B",
volume = "360",
pages = "77",
year = "1995",
author = "T. Reisz",
}

@article{PhysRevE.51.1894,
  author = {Antonenko, S. A. and Sokolov, A. I.},
  journal = {Phys. Rev. E},
  volume = {51},
  issue = {3},
  pages = {1894},
  year = {1995},
}

@article{CAMPOSTRINI1996207,
journal = "Nucl. Phys. B",
volume = "459",
pages = "207",
year = "1996",
author = "M. Campostrini and A. Pelissetto and P. Rossi and E. Vicari",
}

@article{S96,
  title={},
  author={A. I. Sokolov},
  journal={Fiz. Tverd. Tela},
  volume={38},
  pages={640},
  year={1996},
  note={{Sov.} Phys. Sol. State 19 (1996) 354}
}

@article{ZLF,
  author = {Zinn, S.-Y. and Lai, S.-N. and Fisher, M. E.},
  journal = {Phys. Rev. E},
  volume = {54},
  issue = {2},
  pages = {1176},
  year = {1996},
}

@article{SOU,
journal = "Phys. Lett. A",
volume = "227",
pages = "255",
year = "1997",
author = "A.I Sokolov and E.V Orlov and V.A Ul'kov",
}

@article{GZ97,
journal = "Nucl. Phys. B",
volume = "489",
pages = "626",
year = "1997",
author = "R. Guida and J. Zinn-Justin",
}

@article{Morr,
journal = "Nucl. Phys. B",
volume = "495",
pages = "477",
year = "1997",
author = "T. R. Morris",
}

@article{BC97,
  author = {Butera, P. and Comi, M.},
  journal = {Phys. Rev. E},
  volume = {55},
  issue = {6},
  pages = {6391},
  year = {1997},
}

@article{GZJ98,
	year = 1998,
	volume = {31},
	pages = {8103},
	author = {R Guida and J Zinn-Justin},
	journal = {J. Phys. A},
}

@article{SO98,
  author = {Sokolov, A. I. and Orlov, E. V.},
  journal = {Phys. Rev. B},
  volume = {58},
  issue = {5},
  pages = {2395},
  year = {1998},
}

@article{BC98,
  author = {Butera, P. and Comi, M.},
  journal = {Phys. Rev. B},
  volume = {58},
  issue = {17},
  pages = {11552},
  year = {1998},
}

@article{PV,
journal = "Nucl. Phys. B",
volume = "522",
pages = "605",
year = "1998",
author = "A. Pelissetto and E. Vicari",
}

@article{PV98,
journal = "Nucl. Phys. B",
volume = "519",
pages = "626",
year = "1998",
author = "A. Pelissetto and E. Vicari",
}

@article{S98,
  title={},
  author={A. I. Sokolov},
  journal={Fiz. Tverd. Tela},
  volume={40},
  pages={1284},
  year={1998},
  note={{Sov.} Phys. Sol. State 40 (1998) 1169}
}

@article{SOUK99,
  author = {Sokolov, A. I. and Orlov, E. V. and Ul'kov, V. A. and Kashtanov, S. S.},
  journal = {Phys. Rev. E},
  volume = {60},
  issue = {2},
  pages = {1344},
  year = {1999},
}

@article{CPRV99,
  author = {Campostrini, M. and Pelissetto, A. and Rossi, P. and Vicari, E.},
  journal = {Phys. Rev. E},
  volume = {60},
  issue = {4},
  pages = {3526},
  year = {1999},
}

@article{PV2000,
journal = "Nucl. Phys. B",
volume = "575",
pages = "579",
year = "2000",
author = "A. Pelissetto and E. Vicari",
}

@article{PS2000,
  author = {Pakhnin, D. V. and Sokolov, A. I.},
  journal = {Phys. Rev. B},
  volume = {61},
  issue = {22},
  pages = {15130},
  year = {2000},
}

@article{CPV2000,
  author = {Carmona, J. M. and Pelissetto, A. and Vicari, E.},
  journal = {Phys. Rev. B},
  volume = {61},
  issue = {22},
  pages = {15136},
  year = {2000},
}

@article{PS2001,
  author = {Pakhnin, D. V. and Sokolov, A. I.},
  journal = {Phys. Rev. B},
  volume = {64},
  issue = {9},
  pages = {094407},
  year = {2001},
}

@article{ZJ01,
journal = "Phys. Reports",
volume = "344",
pages = "159",
year = "2001",
author = "J Zinn-Justin",
}

@article{CHPV2001,
	year = 2001,
	volume = {34},
	pages = {2923},
	author = {M. Caselle and M. Hasenbusch and A.Pelissetto and E. Vicari},
    journal = {J. Phys. A},
}

@article{CHPRV2001,
  author = {Campostrini, M. and Hasenbusch, M. and Pelissetto, A. and Rossi, P. and Vicari, E.},
  journal = {Phys. Rev. B},
  volume = {63},
  issue = {21},
  pages = {214503},
  year = {2001},
}

@article{CHPRV2002,
  author = {Campostrini, M. and Hasenbusch, M. and Pelissetto, A. and Rossi, P. and Vicari, E.},
  journal = {Phys. Rev. B},
  volume = {65},
  issue = {14},
  pages = {144520},
  year = {2002},
}

@article{CPRV2002,
  author = {Campostrini, M. and Pelissetto, A. and Rossi, P. and Vicari, E.},
  journal = {Phys. Rev. E},
  volume = {65},
  issue = {6},
  pages = {066127},
  year = {2002},
}
@book{ZJ,
  year = {2002},
  publisher = {Oxford University Press},
  author = {J. Zinn-Justin},
  title = {Quantum Field Theory and Critical Phenomena}
}
@article{PV02,
journal = "Phys. Reports",
volume = "368",
pages = "549",
year = "2002",
author = "A. Pelissetto and E. Vicari",
}
@article{TPV03,
	year = 2003,
	volume = {2003},
	pages = {029},
	author = {F. P. Toldin and A. Pelissetto and E. Vicari},
journal = {J. High Energy Phys.},
}
@article{BT2005,
journal = "Nucl. Phys. B",
volume = "704",
pages = "527",
year = "2005",
author = "A. Butti and F. P. Toldin",
}
@article{CSS07,
	year = 2007,
	volume = {40},
	pages = {901},
	author = {D. O'Connor and J. A. Santiago and C. R. Stephens},
}
@article{BP11,
  author = {Butera, P. and Pernici, M.},
  journal = {Phys. Rev. B},
  volume = {83},
  issue = {5},
  pages = {054433},
  year = {2011},
}
@article{NS14,
  author = {Sokolov, A. I. and Nikitina, M. A.},
  journal = {Phys. Rev. E},
  volume = {89},
  issue = {5},
  pages = {052127},
  year = {2014},
}
@article{KKN16,
journal = "Nucl. Phys. B",
volume = "905",
pages = "16",
year = "2016",
author = "G.A. Kalagov and M.V. Kompaniets and M.Yu. Nalimov",
}
@article{KS16,
  author = {Kudlis, A. and Sokolov, A. I.},
  journal = {Phys. Rev. E},
  volume = {94},
  issue = {4},
  pages = {042107},
  year = {2016},
}
@article{K16,
	year = 2016,
	volume = {762},
	pages = {012075},
	author = {M.V. Kompaniets},
	journal = {J. Phys. Conf. Series},
}

@Article{KS17,
author="Kudlis, A.
and Sokolov, A. I.",
journal="Theor. Math. Phys.",
year="2017",
volume="190",
pages="295",
note={Theor. Math. Phys. 176 (2013) 948}
}

@Article{AKL17,
author="Antonov, N. V.
and Kompaniets, M. V.
and Lebedev, N. M.",
journal="Theor. Math. Phys.",
year="2017",
volume="190",
pages="204",
note={Theor. Math. Phys. 176 (2013) 948}
}
@article{SNK17,
journal = "Nucl. Phys. B",
volume = "921",
pages = "225",
year = "2017",
author = "A.I. Sokolov and A. Kudlis and M.A. Nikitina",
}
@article{KP17,
  author = {Kompaniets, M. V. and Panzer, E.},
  journal = {Phys. Rev. D},
  volume = {96},
  issue = {3},
  pages = {036016},
  year = {2017},
}

@article{LK17,
  author = {N. M. Lebedev and M. V. Kompaniets},
  journal = {Vestnik SPbGU, Physics and
Chemistry},
  volume = {4},
  pages = {417},
  year = {2017},
}
@article{FH99,
author = {von Ferber, C. and Holovatch, Yu.},
  journal = {Phys. Rev. E},
  volume = {59},
  issue = {6},
  pages = {6914},
  year = {1999},
}
@article{FHY2000,
  author = {Folk, R. and Holovatch, Yu. and Yavors'kii, T.},
  journal = {Phys. Rev. B},
  volume = {62},
  issue = {18},
  pages = {12195},
  year = {2000},
}

@article{HDY01,
  author = {Yu. Holovatch and M. Dudka and T. Yavorskii},
  journal = {J. Phys. Stud.},
  volume = {5},
  pages = {233},
  year = {2001},
}

@article{DHY02,
  author = {M. Dudka and Yu. Holovatch and T. Yavorskii},
  journal = {Acta Phys. Slov.},
  volume = {52},
  pages = {323},
  year = {2002},
}
@article{CPN04,
journal = "Nucl. Phys. B",
volume = "679",
pages = "568",
year = "2004",
author = "P. Calabrese and P. Parruccini",
}

@article{CP04,
	year = 2004,
	volume = {2004},
	pages = {018},
	author = {P. Calabrese and P. Parruccini},
	journal = {J. High Energy Phys.},
}

@article{COPS04,
  author = {Calabrese, P. and Orlov, E. V. and Pakhnin, D. V. and Sokolov, A. I.},
  journal = {Phys. Rev. B},
  volume = {70},
  issue = {9},
  pages = {094425},
  year = {2004},
}

@article{HID04,
	year = 2004,
	volume = {37},
	pages = {3569},
	author = {Y. Holovatch and D. Ivaneyko and B. Delamotte},
    journal = {J. Phys. A},
}

@article{DHY04,
    year = 2004,
	volume = {37},
	pages = {10727},
	author = {M. Dudka and Y. Holovatch and T. Yavorskii},
	journal = {J. Phys. A},
}

@article{CP05,
  author = {Calabrese, P. and Parruccini, P.},
  journal = {Phys. Rev. B},
  volume = {71},
  issue = {6},
  pages = {064416},
  year = {2005},
}

@article{S2005,
  title={},
  author={A. I. Sokolov},
  journal={Fiz. Tverd. Tela},
  volume={47},
  pages={2056},
  year={2005},
  note={{Sov.} Phys. Sol. State 47 (2005) 2144}
}


@Article{S2013,
author="Sokolov, A. I.",
journal="Teor. Mat. Fiz.",
year="2013",
volume="176",
pages="140",
note={Theor. Math. Phys. 176 (2013) 948}
}

@article{NS13,
  author = {Nikitina, M. A. and Sokolov, A. I.},
  journal = {Phys. Rev. E},
  volume = {89},
  issue = {4},
  pages = {042146},
  year = {2014},
}

@article{NS14e,
  author = {Sokolov, A. I. and Nikitina, M. A.},
  journal = {Phys. Rev. E},
  volume = {90},
  issue = {1},
  pages = {012102},
  year = {2014},
}

@Article{NS16,
author=" M. A. Nikitina and A. I. Sokolov",
journal="Teor. Mat. Fiz.",
year="2016",
volume="186",
pages="230",
note={Theor. Math. Phys. 186 (2016) 192}
}

@article{NS16h,
journal = "Physica A",
volume = "444",
pages = "177",
year = "2016",
author = "A.I. Sokolov and M.A. Nikitina",
}

@article{SS78,
  author = {Sauls, J. A. and Serene, J. W.},
  journal = {Phys. Rev. D},
  volume = {17},
  issue = {6},
  pages = {1524},
  year = {1978},
}


@Article{S80n,
author="A. I. Sokolov",
journal="Zh. Eksp. Teor. Fiz.",
year="1980",
volume="79",
pages="1137",
note={Sov. Phys. JETP 52 (1980) 575}
}

@article{MS73,
  author = {Mermin, N. D. and Stare, C.},
  journal = {Phys. Rev. Lett.},
  volume = {30},
  issue = {22},
  pages = {1135},
  year = {1973},
}

@Article{S80h,
author="A. I. Sokolov",
journal="Zh. Eksp. Teor. Fiz.",
year="1980",
volume="78",
pages="1985",
note={Sov. Phys. JETP 51 (1980) 998}
}

@article{AIKKS,
journal = "Nucl. Phys. B",
volume = "940",
pages = "332",
year = "2019",
author = "L. Ts. Adzhemyan and E. V. Ivanova and M. V. Kompaniets and A. Kudlis and A. I. Sokolov",
}

@article{FH97,
  author = {von Ferber, C. and Holovatch, Yu.},
  journal = {Phys. Rev. E},
  volume = {56},
  issue = {6},
  pages = {6370},
  year = {1997},
 }


